Mechanisms of drag reduction by semi-dilute inertial particles in turbulent channel flow

We investigate the mechanisms by which inertial particles dispersed at semi-dilute conditions cause significant drag-reduction in a turbulent channel flow at $\mathrm{Re}_\tau = 180$. We consider a series of four-way coupled Euler-Lagrange simulations where particles having friction Stokes number $\mathrm{St}^+ = 6$ or 30 are introduced at progressively increasing mass loading from $M=0.2$ to 1.0. The simulations show that $\mathrm{St}^+ = 30$ particles cause large drag-reduction by up to 19.74\% at $M=1.0$, whereas $\mathrm{St}^+ = 6$ particles cause large drag increase by up to 16.92\% at $M=1.0$. To reveal the mechanisms underpinning drag-reduction or drag-increase, we investigate the stress distribution within the channel and the impact of the dispersed particles on the near-wall coherent structures. We find a distinctive feature of drag-reducing particles which consists in the formation of extremely long clusters, called ropes. These structures align preferentially with the low-speed streaks and contribute to their stabilization and suppression of bursting. Despite the additional stresses due to the particles, the modulation of the near-wall coherent structures leads to a greater reduction of Reynolds shear stresses and partial relaminarization of the near-wall flow. In the case of the drag-increasing particles with $\mathrm{St}^+ = 6$, a reduction in Reynolds shear stresses is also observed, however, this reduction is insufficient to overcome the additional particle stresses which leads to drag increase.

==> sections/fluid_particle_interaction.tex <==
\subsection{Particle-fluid interaction}

\begin{figure}[htp]
	\begin{subfigure}{0.45\textwidth}
	    \centering
	    \includegraphics[width=1\linewidth]{plotting/PRE.pdf}
	    \caption{}
	    \label{fig:pre}
	\end{subfigure}
	\begin{subfigure}{0.45\textwidth}
	    \centering
	    \includegraphics[width=1\linewidth]{plotting/PRESCALED.pdf}
	    \caption{}
	    \label{fig:pre_scaled}
	\end{subfigure}		
	\caption{Particle Reynolds number shows that within the log-layer region and even further away from it particles do present a wake and influence the flow around them.}
	\label{fig:pre_stats}
\end{figure} 

Particle Reynolds number, $\Rey_p$ is a good parameter to understand how particles modulate the flow based on their physical properties (i.e. particle diameter, Stokes number and particle density). We begin investigating this particle-phase of the channel flow by measuring the particle Reynolds number, $\Rey_p$ within the flow. Figure \ref{fig:pre} shows that $\Rey_p$ is the highest in the log-layer region. It is known from theory \citep{bagchiDirectNumericalSimulation2001}\citep{richterDragForcesHeat2012} that as $\Rey_p$ increases particles create a greater wake, affecting fluid statistics and also nearby particle movement, especially within the log layer maximum flux in all quantities is observed. Furthermore, for the $\Rey_p$ range observed within fig. \ref{fig:pre}, it is inferred that the drag law proposed by \citet{tennetiDragLawMonodisperse2011a} is appropriate. 

To further understand the modulation of the mean streamwise velocity $U_f^+$, \ref{fig:pre_scaled} shows the scaled particle Reynolds number, $\Rey_p/\sqrt{\Sto^+}$. All cases seem to collapse closely, with case \textbf{C} and \textbf{F} showung a slight increase in the log layer region. This is in line with what is witnessed in fig. \ref{fig:fvelst6} and \ref{fig:fvelst30}, showing that it is the slip velocity that controls the intensity of the modulation performed on the fluid by the inertial particles. However, it is the inertia that control whether we see an increase or decrease in the mass flow rate. The higher the slip velocity within the log layer, the greater the modulation. Figure \ref{fig:fvel} shows that case \textbf{C} has masximum drag and also consequently has the highest slip velocity for particles at $\Sto^+ = 6$. Case \textbf{F} on the other hand mas maximum mass flow rate recorded and consequently also has the higher slip velocity recorded in the log region for particles with $\Sto^+ = 30$.

\begin{figure}[htp]
  \begin{subfigure}{0.8\textwidth}
    \centering
    \includegraphics[width=1\linewidth,trim={0ex 8ex 0ex 8ex},clip]{images/vfp_s6m02.png}
    \caption{$ St^+ = 6, M = 0.2$}
    \label{fig:vfp_s6m02}
  \end{subfigure}
  \begin{subfigure}{0.8\textwidth}
    \centering
    \includegraphics[width=1\linewidth,trim={0ex 8ex 0ex 8ex},clip]{images/vfp_s6m04.png}
    \caption{$St^+ = 6, M = 0.4$}
    \label{fig:vfp_s6m04}
  \end{subfigure}
  \begin{subfigure}{0.8\textwidth}
    \centering
    \includegraphics[width=1\linewidth,trim={0ex 8ex 0ex 8ex},clip]{images/vfp_s6m06.png}
    \caption{$St^+ = 6, M = 0.6$}
    \label{fig:vfp_s6m06}
  \end{subfigure}
  \begin{subfigure}{0.8\textwidth}
    \centering
    \includegraphics[width=1\linewidth,trim={0ex 8ex 0ex 8ex},clip]{images/vfp_s30m02.png}
    \caption{$St^+ =30, M = 0.2$}
    \label{fig:vfp_s30m02}
  \end{subfigure}
  \begin{subfigure}{0.8\textwidth}
    \centering
    \includegraphics[width=1\linewidth,trim={0ex 8ex 0ex 8ex},clip]{images/vfp_s30m04.png}
    \caption{$St^+ =30, M = 0.4$}
    \label{fig:vfp_s30m04}
  \end{subfigure}
  \begin{subfigure}{0.8\textwidth}
    \centering
    \includegraphics[width=1\linewidth,trim={0ex 8ex 0ex 8ex},clip]{images/vfp_s30m06.png}
    \caption{$St^+ =30, M = 0.6$}
    \label{fig:vfp_s30m06}
  \end{subfigure}
  \caption{Particle volume fraction normalized by the average volume fraction showing formation of clusters within the flow in high strain regions and the accumalation of particles near the wall through turbophoresis}
  \label{fig:vfp}
\end{figure}

Particle laden flows with a semi-dilute concentration have a substantial effect on fluid characteristics mainly due to two phenomenons that take place simultaneously within a particle-laden flow. Preferential concentration ejects particles from high vorticity (low strain) regions towards low vorticity (high strain) regions of the flow. This can help remove energy from these high vorticity regions as they get ejected outwards. Moreover, the effect of turboproresis near the wall allows for particles to segregate much closer to the wall with time as the the flow is driven within the channel. This effect of turbophoresis that aids in a higher localized volume fraction near the wall increases the effect of preferential concentration aiding in formations of clusters near the wall. To further take a look into this effect fig. \ref{fig:vfp} shows the particle volume fraction normalized by its average volume fraction and fig. \ref{fig:pnd} shows the particle number density relative to their distance from the wall.
      
\begin{figure}[htp]
    \centering
    \includegraphics[scale=0.5]{plotting/PND.pdf}
    \caption{Particle number density does not show strong dependence on mass loading in the semi-dilute regime as we can see all cases closely resembling each other apart from near the wall where we see maximum accumalation of particler as $\Sto^+$ increases.}
    \label{fig:pnd}
\end{figure}  

All cases show the effects of turbophoresis where maximum accumalation is observed near the wall however, heavier particles (i.e. larger Stokes numbers) tend to stay closer to the wall compared to lighter particles (i.e. smaller Stokes numbers). Previous studies by \citet{sardinaWallAccumulationSpatial2012} show greater accumalation of inertial particles near the wall as the Stokes number is increased. Figure \ref{fig:vfp} shows dense clustering within the channel as the mass loading is increased. Large particle clusters are observed near the wall for cases \textbf{D}, \textbf{E} and \textbf{F} compared to the center of the flow because of their high inertia. Contrastingly cases \textbf{A}, \textbf{B} and \textbf{C} show greater ejection of particles towards the center of the channel by vortical structures away from the wall owing to lower inertia. The length scales of the clusters for particles of $\Sto^+  =6$ stay consistent throughout the channel and become denser as the mass loading is increased, while the length scales for particles of $\Sto^+ = 30$ are higher near the wall than in the center of the flow and become denser as the mass loading is increased. This behaviour can be further witnessed in figure \ref{fig:pnd}. $\Sto^+ = 30$ cases show greater particle number density near the wall compared to $\Sto^+ = 6$ while having lesser particle number density away from the wall. It can therefore be hypothesized that larger Stokes numbers modulate the fluid largely near the wall while smaller Stokes numbers modulate the flow in all regions of the channel. This is consistent from trends we have seen in previous studies by \citet{fongVelocitySpatialDistribution2019}. Particles of $\Sto^+$ of O(10) display greater modulation of the fluid compared to particles of $\Sto^+$ of O(1) because of the large macro-scale focres they apply on the fluid due to the dense clustering near the wall.

\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{images/3driblet.png}
    \caption{Particles forming large riblets throughout the channel at high Stokes numbers ($\Sto^+ = 30, M = 0.6$}
    \label{fig:3driblet}
\end{figure}

To further understand the movement of oartucles near the wall and how inertia and mass loading affect the clustering, a detailed picture is shown in figure \ref{fig:3driblet} and \ref{fig:riblet_comparison}. Figure \ref{fig:3driblet} shows long riblets of particles forming near the wall for case \textbf{F}. Previous experiments have shown that particles arrange themselved in low-speed regions of the flow near the wall. Figure \ref{fig:riblet_comparison} shows the contours of the particles volume fraction for all cases (3 times the average volume fraction for particles of $\Sto^+ = 6$ and 5 times the average volume fraction for particles of $\Sto^+ = 30$) near the wall over the fluid streamwise velocity. The effect of preferential concentration is very evident in all cases \textbf{A}-\textbf{F}. Particles tend to get ejected from high speed (high vorticity) regions to low speed (low vorticity) regions. FOr particles of $\Sto^+ = 6$ (fig. \ref{fig:nribletS6M02}, \ref{fig:nribletS6M04} and \ref{fig:nribletS6M06}), a large number of low-speed regions are present with small clustering of particles near the wall within all these low-speed regions. This is due to the low inertia of the particles, making them `lighter' and allowing them to drift with more ease. Even though, the effect of preferential concentration is evident for particles at $\Sto^+ = 6$, they seem to have a higher level of movement near the wall. This shows that the fluid is strongly modulating the particles, just as equally as the particles are modulating the fluid near the wall when inertia is low. Contrastingly, cases at $\Sto^+ = 30$ show longer more well defined low-speed regions. Particles have larger clusters, multiple length scales bigger than particle clusters at $\Sto^+ = 6$. As the mass loading is increased the long particle clusters (i.e. `riblets') become more defined (fig. \ref{fig:nribletS30M06}). A three dimentional representation of that is shown in fig. \ref{fig:3driblet}. Low speed regions become thinner but also longer (spanning the entire domain). This is consistent with data on particle-laden flows with larger inertia particles. They tend to be more `heavier', meaning less movement near the wall. However the effect of preferential concentration is still visible with particles forming long riblets within the low speed regions, with minimal to almost non in the high speed regions. For particle-laden cases at $\Sto^+ = 30$, there are relatively less number of particle clusters but longer clusters than flows with inertial particles at $\Sto^+ = 6$. Fewer clustering means fewer movement of particles in and out of different vorticity regions of the flow. The particles tend to modulate the fluid more stronglt than the fluid modulating the particles for higher inertia particle-laden cases.   

\begin{figure}[htp]
  \begin{subfigure}{0.75\textwidth}
    \centering
    \includegraphics[width=1\linewidth,trim={0ex 8ex 0ex 8ex},clip]{images/nribletS6M02.png}
    \caption{$ \Sto^+ = 6, M = 0.2$}
    \label{fig:nribletS6M02}
  \end{subfigure}
  \begin{subfigure}{0.75\textwidth}
    \centering
    \includegraphics[width=1\linewidth,trim={0ex 8ex 0ex 8ex},clip]{images/nribletS6M04.png}
    \caption{$\Sto^+ = 6, M = 0.4$}
    \label{fig:nribletS6M04}
  \end{subfigure}
  \begin{subfigure}{0.75\textwidth}
    \centering
    \includegraphics[width=1\linewidth,trim={0ex 8ex 0ex 8ex},clip]{images/nribletS6M06.png}
    \caption{$\Sto^+ = 6, M = 0.6$}
    \label{fig:nribletS6M06}
  \end{subfigure}
  \begin{subfigure}{0.75\textwidth}
    \centering
    \includegraphics[width=1\linewidth,trim={0ex 8ex 0ex 8ex},clip]{images/nribletS30M02.png}
    \caption{$\Sto^+ =30, M = 0.2$}
    \label{fig:nribletS30M02}
  \end{subfigure}
  \begin{subfigure}{0.75\textwidth}
    \centering
    \includegraphics[width=1\linewidth,trim={0ex 8ex 0ex 8ex},clip]{images/nribletS30M04.png}
    \caption{$\Sto^+ =30, M = 0.4$}
    \label{fig:nribletS30M04}
  \end{subfigure}
  \begin{subfigure}{0.75\textwidth}
    \centering
    \includegraphics[width=1\linewidth,trim={0ex 8ex 0ex 8ex},clip]{images/nribletS30M06.png}
    \caption{$\Sto^+ =30, M = 0.6$}
    \label{fig:nribletS30M06}
  \end{subfigure}
  \caption{Particle volume fraction (i.e. 3 times the average for (a)(b) and (c) and 5 times the average for (d)(e) and (f)) plotted over the streamwise velocity showing low speed streaks in the fluid, and preferential concentration of particles into these low speed regions creating long riblet like formations for particles at $\Sto^+ = 30$}
  \label{fig:riblet_comparison}
\end{figure}


==> sections/fluid_vel_stats.tex <==
\subsection{Velocity modulation due to particle-fluid interaction}

There has been considerable interest in recent years on drag modulation due to particles within a channel flow. Many studies have been performed using various methods such as the eulerian-lagrangian point particle method \citep{zhouNonmonotonicEffectMass2020,LagrangianStatisticsTurbulent1995,bakerDirectComparisonEulerian2020}, the immersed boundary approach \citep{picanoTurbulentChannelFlow2015,breugemSecondorderAccurateImmersed2012} and the lattice Boltzmann method \citep{pengDirectNumericalInvestigation2019,wangLatticeBoltzmannSimulation2016,zhangLatticeBoltzmannMethod2016}. Studies however have not been able to present a clear picture as to how different particle characteristics (Stokes number, mass loading) affect the drag within a flow. This section aims to understand the velocity statistics for low-moderate mass loading (0.2-0.6) at Stokes numbers of O(1-10) [Cases \textbf{A-C} ($\Sto^+ = 6$) and cases \textbf{D-F} ($\Sto^+ = 30$)], using the eulerian-lagrangian point particle approach, which has been a proven method for particle-laden flows (**reference needed**). 

\begin{figure}[htp]
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{plotting/AVGVEL_ST6.pdf}
    \caption{}
    \label{fig:fvelst6}
  \end{subfigure}
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{plotting/FURMS_ST6.pdf}
    \caption{}
    \label{fig:furmsst6}
  \end{subfigure}
  \caption{(a) Streamwise velocity and (b) streamwise velocity fluctuations plotted as a function of $y^+$ for $St^+ = 6$.} 
  \label{fig:fluid_stats_st6}
\end{figure}

\begin{figure}[htp]
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{plotting/AVGVEL_ST30.pdf}
    \caption{}
    \label{fig:fvelst30}
  \end{subfigure}
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{plotting/FURMS_ST30.pdf}
    \caption{}
    \label{fig:furmsst30}
  \end{subfigure}
  \caption{(a) Streamwise velocity and (b) streamwise velocity fluctuations plotted as a function of $y^+$ for $St^+ = 30$.} 
  \label{fig:fluid_stats_st30}
\end{figure}

Figure \ref{fig:fluid_stats_st6} shows the streamwise velocity $\langle u_f\rangle / u_\tau$ and the streamwise fluctuations $\sqrt{\langle u^{`2}_f \rangle}/u_\tau$ for cases \textbf{A-C}. It is observed that the particles have a weak modulation on the near wall statistics for for $\langle u_f\rangle / u_\tau$ and $\sqrt{\langle u^{`2}_f \rangle}/u_\tau$ at $\Sto^+ = 6$. There is a monotonic reduction observed for $\langle u_f\rangle / u_\tau$ in the outer layer with increasing mass loading. $\sqrt{\langle u^{`2}_f \rangle}/u_\tau$ decreases throughout the channel compared to the single phase flow, with maximum modulation witnessed for case \textbf{C}. 

Cases \textbf{D-F} all present an enhancement in $\langle u_f\rangle / u_\tau$ with maximum increase observed for case \textbf{F} as shown in fig. \ref{fig:fvelst30}. \citet{zhouNonmonotonicEffectMass2020} conduct a similar study as shown for cases \textbf{D-F} at $\Rey_\tau = 180$ and $\Sto^+ = 30$. They observe a similar increase in $\langle u_f\rangle / u_\tau$ within the log-outer layer, with the exception that the present study does not observe the near center-line reduction that was witnessed by \citet{zhouNonmonotonicEffectMass2020}. There is a significant near-wall reduction in $\sqrt{\langle u^{`2}_f \rangle}/u_\tau$, and a monotonic increase in the log-outer layer with increasing mass loading for cases \textbf{D-F} as shown in fig. \ref{fig:furmsst30}. A similar behaviour was observed by \citet{zhouNonmonotonicEffectMass2020}. 

The modulation of the streamwise velocity fluctuations, more specifically within the log-outer layer show a direct correlation to the increase in the overall mass flow rate. As the log-outer layer $\sqrt{\langle u^{`2}_f \rangle}/u_\tau$ is decreased we see a reduction in the mass flow rate (cases \textbf{A-C}),  and as $\sqrt{\langle u^{`2}_f \rangle}/u_\tau$ is increased in the log-outer layer we see an increase in the mass flow rate (cases \textbf{D-F}). 

The wall normal (fig. \ref{fig:fvrms}) and spanwise (fig. \ref{fig:fwrms}) velocity fluctuations show a significant reduction within the flow for all cases compared to the single phase flow. There is a strong relationship between increasing mass loading and decreasing $\sqrt{\langle v^{`2}_f \rangle}/u_\tau$ and $\sqrt{\langle w^{`2}_f \rangle}/u_\tau$ within the range of $\Sto^+ = 6-30$. A similar reduction is also noticed by \citet{zhouNonmonotonicEffectMass2020}, for particle-laden channel flows run at a similar semi-dilute regime at $St^+ = 30$. The mass loading therefore plays a more significant role than the Stokes number in modulating the fluid wall-normal and spanwise velocity fluctuations in a semi-dilute regime in the range of $St^+ = O(1-10)$. 

The modulation of the streamwise fluid velocity within the channel is therefore dependent largely on the streamwise velocity fluctuations. Enhancement of the mass flow rate can be achieved through particles that have a higher inertia ($\Sto^+ = 30$), due to staying closer to the wall. This helps modulate the fluid characteristics near the wall more strongly, primarily $\sqrt{\langle u^{`2}_f \rangle}/u_\tau$,  than particle with a lower inertia ($\Sto^+ = 6$). Particles with a larger inertia tend to stay closer to the wall on average throughout the channel compared to lower inertia paticles which are more spread out within the channel. This is shown clearly in fig. \ref{fig:pnd}, where the particle number density is plotted compared to the distance away from the wall. From fig. \ref{fig:fluid_stats_st6}, \ref{fig:fluid_stats_st30} and \ref{fig:fluid_stats_rms}, we can notice that particles help reduce the velocity fluctuations around them. However, it is observed that greater log-outer layer streamwise fluid velocity fluctuations helps aid the enhancement in the mass flow rate. This is easier done through particles of higher inertia that stay closer to the wall reducing the near wall streamwise fluid fluctuations significantly increasing the log-outer layer fluctuations, enhancing the overall mass flow rate. In contrast lower inertia particles tend to be scattered throughout the channel, not delivering the effect that higher inertia particles do in modulation the fluid flow.       

\begin{figure}[htp]
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{plotting/FVRMS.pdf}
    \caption{}
    \label{fig:fvrms}
  \end{subfigure}
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{plotting/FWRMS.pdf}
    \caption{}
    \label{fig:fwrms}
  \end{subfigure}
  \caption{(a) Wall-normal and (b) spanwise fluctuations plotted as a function of $y^+$.} 
  \label{fig:fluid_stats_rms}
\end{figure}

The present study aims to understand the behaviour of the particle phase compared to the fluid phase as we move away from the wall. Figure \ref{fig:fluid_particle_vel_stats}, \ref{fig:global_fluid_particle_velfluc_stats} and \ref{fig:pc_fluid_particle_velfluc_stats} take a look at the velocity characteristics between the two phases to understand how particle help modulate the fluid due to turbophoresis and preferential concentration. Figure \ref{fig:fluid_particle_vel_stats} compares the streamwise velocity between the particle $\langle u_p \rangle/u_\tau$ and the fluid $\langle u_f \rangle/u_\tau$ phase. Additionally, the fluid streamwise velocity conditioned at particle locations $\langle u_{f\mid p}\rangle/u_\tau$ is also presented. From all the cases it is observed that higher inertial particles ($\Sto^+ = 30$) modulate the fluid by showing a greater streamwise velocity within all regions of the flow i.e. $\langle u_f \rangle/u_\tau$, $\langle u_p \rangle/u_\tau$ and $\langle u_{f\mid p}\rangle/u_\tau$ compared to lower inertial particles ($\Sto^+ = 6$). Furthermore, All particle-laden cases show a similar behaviour overall with the particle phase lagging the fluid phase in the near-wall region. As the mass loading is increased the near wall streamwise velocity difference between the particle phase and the fluid phase is increased. However, the fluid at the particle locations significantly lags the overall flow. The magnitude of $\langle u_{f\mid p}\rangle/u_\tau$ is dependent on the inertia of the particles. Cases \textbf{D-F} show a higher $\langle u_{f\mid p}\rangle/u_\tau$ compared to cases \textbf{A-C} within all layers of the turbulent boundary layer and within the outer region.     

\begin{figure}[htp]
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{plotting/FPFPLU02.pdf}
    \caption{M = 0.2}
    \label{fig:fpfplu02}
  \end{subfigure}
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{plotting/FPFPLU02.pdf}
    \caption{M = 0.4}
    \label{fig:fpflpu04}
  \end{subfigure}
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{plotting/FPFPLU06.pdf}
    \caption{M = 0.6}
    \label{fig:fpflpu06}
  \end{subfigure}
  \caption{Fluid particle velocity comparison} 
  \label{fig:fluid_particle_vel_stats}
\end{figure}

To understand the particle modulation on the fluid further, fig. \ref{fig:global_fluid_particle_velfluc_stats} takes a look at the global fluid and particle velocity fluctuations in comparison. Figure \ref{fig:pfurms_st6} (\textbf{A-C}) and \ref{fig:pfurms_st30} (\textbf{D-F}) show the streamwise velocity fluctuations comparison between the particle and fluid phase. It is observed for the streamwise velocity fluctuations that the particle phase leads the fluid in the near wall region and lags the fluid in the outer layer for all inertial particles. Mass loading does not play a significant role in the modulation of the streamwise velocity fluctuations for particles of inertia $\Sto^+ = 6$, however as the inertia is increased there is monotonic increase in the fluid and particle streamwise velocity fluctuations as the mass loading is increased. The wall normal (fig. \ref{fig:pfvrms_st6},\ref{fig:pfvrms_st30}) and spanwise (fig. \ref{fig:pfwrms_st6},\ref{fig:pfwrms_st30}) velocity fluctuations on the other hand, both have the particle phase lagging the fluid phase and mass loading plays a role for all inertial particles. There is a monotonic decrease in both the fluid and particle wall normal and spanwise velocity fluctiations as mass loading is increased.    

\begin{figure}[htp]
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{plotting/PFURMS_ST6.pdf}
    \caption{$St^+ = 6$}
    \label{fig:pfurms_st6}
  \end{subfigure}
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{plotting/PFURMS_ST30.pdf}
    \caption{$St^+ = 30$}
    \label{fig:pfurms_st30}
  \end{subfigure}
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{plotting/PFVRMS_ST6.pdf}
    \caption{$St^+ = 6$}
    \label{fig:pfvrms_st6}
  \end{subfigure}
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{plotting/PFVRMS_ST30.pdf}
    \caption{$St^+ = 30$}
    \label{fig:pfvrms_st30}
  \end{subfigure}
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{plotting/PFWRMS_ST6.pdf}
    \caption{$St^+ = 6$}
    \label{fig:pfwrms_st6}
  \end{subfigure}
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{plotting/PFWRMS_ST30.pdf}
    \caption{$St^+ = 30$}
    \label{fig:pfwrms_st30}
  \end{subfigure}
  \caption{Global fluid particle velocity fluctuations comparison} 
  \label{fig:global_fluid_particle_velfluc_stats}
\end{figure}

The modulatin of the fluid velocity fluctuations by the particles is better understood by taking a look at the fluid velocity fluctuations at particle locations. Figure \ref{fig:pc_fluid_particle_velfluc_stats} shows the particle velocity fluctuations and the fluid velocity fluctuations at the particle locations. The reduction in the near-wall fluid streamwise velocity fluctuations $\sqrt{\langle u^{`2}_f \rangle}/u_\tau$, is due to the partiles modulating the fluid significantly. $\sqrt{\langle u^{`2}_{f \mid p} \rangle}/u_\tau$ is notably reduced near the wall (i.e. fig. \ref{fig:pcpfurms_st6}, \ref{fig:pcpfurms_st30}), helping reduce the overall $\sqrt{\langle u^{`2}_f \rangle}/u_\tau$ in that region. As observed in fig. \ref{fig:global_fluid_particle_velfluc_stats}, $\sqrt{\langle v^{`2}_p \rangle}/u_\tau$ and $\sqrt{\langle w^{`2}_p \rangle}/u_\tau$ have always been lower than the fluid counterpart. Furthermore, these particles tend to modulate the fluid strongly by reducing the $\sqrt{\langle v^{`2}_f \rangle}/u_\tau$ and $\sqrt{\langle w^{`2}_f \rangle}/u_\tau$ compared to the single phase flow. This modulation is better observed in fig. \ref{fig:pcpfvrms_st6}, \ref{fig:pcpfvrms_st30} (wall-normal velocity fluctuations) and fig. \ref{fig:pcpfwrms_st6}, \ref{fig:pcpfwrms_st30} (spanwise velocity fluctuations). The particles help significantly reduce the fluid velocity fluctuations at particle locations. This in turn helps reduce the global fluid velocity fluctuations. A common observation across all particle-laden cases is that the near-wall modulation of the fluid is stronger than the outer layer modulation. This is due to turbophoresis pushing the majority of the particles closer to the wall. Particles with a higher inertia ($St^+ = 30 > St^+ = 6$) tend to be 'heavier' and stay closer to the wall modulating the fluid more strongly. Figures \ref{fig:fluid_stats_st6} - \ref{fig:pc_fluid_particle_velfluc_stats} show that the more the near-wall $\sqrt{\langle u^{`2}_f \rangle}/u_\tau$ is reduced (in turn increasing the log-outer layer $\sqrt{\langle u^{`2}_f \rangle}/u_\tau$), the stronger the increase in the mass flow rate. Particles with a higher Stokes number tend to be able to perform better in increasing the mass flow rate because they tend the modulate the near-wall statistics more strongly that lower Stokes number particles. On the other hand, lower Stokes number particles tend to modulate the flow weakly throughout the channel, but also tend to modulate the flow in regions (i.e. log-outer layer) where drag enhancement is produced.    

\begin{figure}[htp]
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{plotting/PC_PFURMS_ST6.pdf}
    \caption{$St^+ = 6$}
    \label{fig:pcpfurms_st6}
  \end{subfigure}
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{plotting/PC_PFURMS_ST30.pdf}
    \caption{$St^+ = 30$}
    \label{fig:pcpfurms_st30}
  \end{subfigure}
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{plotting/PC_PFVRMS_ST6.pdf}
    \caption{$St^+ = 6$}
    \label{fig:pcpfvrms_st6}
  \end{subfigure}
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{plotting/PC_PFVRMS_ST30.pdf}
    \caption{$St^+ = 30$}
    \label{fig:pcpfvrms_st30}
  \end{subfigure}
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{plotting/PC_PFWRMS_ST6.pdf}
    \caption{$St^+ = 6$}
    \label{fig:pcpfwrms_st6}
  \end{subfigure}
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{plotting/PC_PFWRMS_ST30.pdf}
    \caption{$St^+ = 30$}
    \label{fig:pcpfwrms_st30}
  \end{subfigure}
  \caption{Fluid conditioned at particle locations and the particle phase velocity fluctuations comparison} 
  \label{fig:pc_fluid_particle_velfluc_stats}
\end{figure}




==> sections/rss_tke.tex <==
\subsection{Contribution to Reynolds shear stress and fluid turbulent kinetic energy}

The contribution to the total shear stress by the Reynolds shear stress $-\rho_f \langle uv \rangle $, and the viscous shear stress $\mu du_{f}/dy$ within wall bounded flows has been of vital importance to understanding the modulation of the mass flow rate within a single phase flows. Through Reynolds averaging, previous studies have arrived on a single equation that describes the turbulent shear stress profile as shown below in eqn. \ref{eq:RSS_1}. Here the total shear stress $\tau$ is shown as the viscous shear stress $\mu\partial u_f/\partial y$ minus the Reynolds shear stress $\rho\langle u_{f}^{'}v_{f}^{'}\rangle$. $\tau$ here as shown by eqn. \ref{eq:RSS_1} has a constant slope as the distance away from the wall.

\begin{equation}
    -\frac{\partial \langle P \rangle}{\partial x} = \frac{\partial}{\partial y}\left(\mu\frac{\partial u_f}{\partial y} - \rho\langle u_{f}'v_{f}'\rangle\right)
    \label{eq:RSS_1}
\end{equation}

The total shear stress, $\tau$ and the contributions to it (viscous and Reynolds stress) for the single phase channel flow is shown in fig. \ref{fig:tss_sp}. It is clear how $\tau$ has a constant slope from the wall to the center of the flow. The viscous shear stress dominates the near wall region, while as we move away from the wall it tends to exponentially decrease in magnitude. Comparatively, the Reynolds shear stress shows the maximum magnitude in the log layer of the flow, and has a steady reduction as we approach the center of the channel.

\begin{figure}[htp]
    \centering
    \includegraphics[width=\linewidth]{plotting/TSS-SP.pdf}
    \caption{Contribution of the Reynolds shear stress and viscous shear stress to the total shear stress within a single phase channel flow.}
    \label{fig:tss_sp}
\end{figure}

However for the current multiphase (particle-laden) cases, The total shear stress is a contribution of the viscous and Reynolds shear stress, and an additional third term, the particle shear stress. This is due to the extra particle momentum exchange term we see added to the conservation of momentum equation in eqn. \ref{eq:NVS_2}. Performing a similar Reynolds averaging on the particle term $\langle F_p \rangle $ yields a similar equation as eqn. \ref{eq:RSS_1} with an extra particle shear stress term as shown in eqn. \ref{eq:RSS_2}. Keep in mind for constant pressure gradient flows (the force driving the flow for all simulations conducted in this study), the integral of the left hand side of the equation $\partial\langle P\rangle/\partial x$, always remains the same, since the pressure gradient forcing is a constant value. Therefore it is of importance to understand how the viscous, Reynolds and particle shear stress curves are modulated within the flow as Stokes number or the mass loading is varied.

\begin{equation}
    -\frac{\partial \langle P \rangle}{\partial x} = \frac{\partial}{\partial y}\left(\mu\frac{\partial u_f}{\partial y} - \rho\langle u_{f}'v_f'\rangle - m_{p}\langle n_{d} \rangle \langle u_{p}'v_{p}' \rangle \right)
    \label{eq:RSS_2}
\end{equation}

From eqn. \ref{eq:RSS_2}, it is observed that the fluid Reynolds shear stress and the particle shear stress are both subtracted from the viscous shear stress. The fluid Reynolds shear stress and particle shear stress therefore, perform a similar role in affecting the total shear stress within a flow. Previous single phase studies have shown that the Reynolds shear stress is a good indicator of the skin-friction drag near the wall. Reducing the magnitude of the Reynolds shear stress can strongly aid in the reduction of the drag experienced by the fluid and increase the mass flow rate. Therefore, we can hypothesize that if the total contribution of $\rho\langle u_{f}^{'}v_{f}^{'}\rangle$ and $m_{p}\langle n_{d} \rangle \langle u_{p}^{'}v_{p}^{'} \rangle$ if lower than the single phase $\rho\langle u_{f}^{'}v_{f}^{'}\rangle$, we can achieve increase in mass flow rate.  

\begin{figure}[htp]
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{plotting/TSS_COMPARE-S6M06.pdf}
    \caption{$\Sto^+ = 6, M = 0.6$}
    \label{fig:tsscomparest6}
  \end{subfigure}
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{plotting/TSS_COMPARE-S30M06.pdf}
    \caption{$\Sto^+ = 30, M = 0.6$}
    \label{fig:tsscomparest30}
  \end{subfigure}
  \caption{This figure shows the shear stress profile for (a) case \textbf{C} (maximum drag enhancement) and (b) case \textbf{F} (maximum drag reduction), compared to the single phase flow (dashed lines) where (\sampleline{dash pattern=on .7em off .2em on .2em off .2em}) is the total shear stress, (\sampleline{dotted}) is the Reynolds shear stress and (\sampleline{dashed}) is the viscous shear stress} 
  \label{fig:tss_comparison}
\end{figure}

Figure \ref{fig:tss_comparison} shows the stress profile and how the different shear stress terms vary in comparison to the single phase flow. As shown in eqn. \ref{eq:RSS_2} The total shear stress profile will always remain the same. Equation \ref{eq:RSS_2} shows that the particle shear stress and the Reynolds shear stress both produce a similar effect as both are subtracted from the viscous shear stress. Therefore, if the viscous stress is increased, the Reynolds and particle stresses should reduce to satisfy eqn. \ref{eq:RSS_2}. Moreover, we know through previous studies (** insert reference) that as the Reynolds shear stress is reduced there is an improvement in the mass flow rate of the fluid. The near coherent structures are responsible for nearly half of the skin friction drag (Guala, JFM, 2006). Modulating these coherent structures can help reduce the skin-friction drag induced within the flow. Figure \ref{fig:tsscomparest30} shows the stress profile for case \textbf{F} and it is observed that the near wall viscous shear stress profile is higher than that of the single phase. This shows that the higher inertial particles help reduce the Reynolds shear stress, and they themselves induce a lower magnitude of stress. This shows how higher inertial particles can help reduce the induced drag and enhance the mass flow rate by modulating the coherent structures near the wall. They can help reduce the Reynolds shear stress significantly while also keeping the particle shear stress low near the wall such that the sum of the Reynolds and particle shear stress near the wall is lower than the Reynolds shear stress of the single phase flow near the wall. Contrastingly, fig. \ref{eq:tsscomparest6} shows the stress profile for lower inertial particles i.e. case \textbf{C}. The near wall viscous stress profile is almost similar to the single phase case. This means that the sum of the Reynolds and particle shear stress are also equal to the single phase Reynolds shear stress near the wall. Case \textbf{C} shows maximum drag enhancement, this is mostly due to the log-outer layer increase in the particle shear stress, due to a large amount of particles being easily ejected into the middle of the channel slowing down the fluid as a result of this.        

To further understand the modulation of the coherent structures near the wall, the Q-criterion is explored to understand how particles modulate the vortical structures near the wall with changing Stokes number while keeping the mass loading the same. The vortical structures are diminished with time as particles are injected into the system. Inertial particles of $\Sto^+$ of O(10) diminish the vortical structures and modulate the fluid significantly more than particles of $\Sto^+$ of order O(1) as we can see in \ref{fig:qcrit}. Further demonstrating how particle-laden flows do not follow the same rules as unladen flows. Diminishing the vortical structures is not the only essential criteria to decreasing the drag of the system. From the results in fig. \ref{fig:fvelst30} and \ref{fig:tsscomparest30} for higher inertia cases and fig. \ref{fig:fvelst6} and \ref{fig:tsscomparest6} for lower inertia cases, it is observed that the mass flow rate of the fluid is not solely dependent on the diminishing of the coherent structures, but also keeping the particle induced shear stress low enough which higher inertial particles perform better at than lower inertial particles. 

\begin{figure}[htp]
    \centering
    \includegraphics[width=\linewidth]{tikzgraphics/q-crit.pdf}
    \caption{The Q-criterion represents the vortical structures near the wall and is a good depiction of thje Reynolds shear stress modulation near the wall. The figure shows that the vortical structures are diminished for all particle-laden cases with higher inertia particles performing better at diminishing these structres than lower inertia particles.}
    \label{fig:qcrit}
\end{figure}

\par
Another phenomenon that can be explored is preferential concentration and how particles transfer the turbulent energy within the flow. Quadrant analysis \citep{wallaceWallRegionTurbulent1972}\citep{adrianStochasticEstimationOrganized1988} was therefore performed on all cases further understand this. The velocity fluctuations within the flow are divided in 4 quadrants based on their signs, where Q1($+u$,$+v$) and Q3($-u$,$-v$) are the outward and inward motions within the flow which dont reveal much about the vortical structures within the flow. Additionally Q2($-u$,$+v$) and Q4($+u$,$-v$) are the ejection and sweep events which reveal the vortical motions within the flow and are the greatest contributors of Reynolds shear stress within the flow. We can observe from fig. \ref{fig:quadrant} for all $\Sto^+ = 6$ and $\Sto^+ = 30$ cases that as the mass loading is increased and more particles are injected within the system we see a monotonic behaviour that depicts a decrease in the Reynolds shear stress contribution by the Q2 and Q4 events which are the sweep and ejection events and also agree with the previous results shown in fig. \ref{fig:tss_comparison}. Furthermore, looking at the sweep and ejection quadrants further confirms what is observed in fig. \ref{fig:tss_comparison}. The log scale graph shows that for the highest mass loading (maximum modulation), the near wall Reynolds stress reduction is more significant for $\Sto^+ = 30$ than for $\Sto^+ = 6$.    

\begin{figure}%[htp]
  \begin{subfigure}{0.45\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{plotting/Q1.pdf}
    \caption{Quadrant 1}
    \label{fig:q1}
  \end{subfigure}
  \begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{plotting/Q2.pdf}
    \caption{Quadrant 2}
    \label{fig:q2}
  \end{subfigure}
  \begin{subfigure}{0.45\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{plotting/Q3.pdf}
    \caption{Quadrant 3}
    \label{fig:q3}
  \end{subfigure}
  \begin{subfigure}{0.45\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{plotting/Q4.pdf}
    \caption{Quadrant 4}
    \label{fig:q4}
  \end{subfigure}
  \caption{Quadrant analysis for all cases normalized by ${u_\tau}^2$ as a function of $y^+$. The results agree very well to literature where we see the maximum contribution to the Reynolds stress is due to Q2 and Q4.}
  \label{fig:quadrant}
\end{figure}

~

